Angular distribution of $\Lambda_b^0\to pK^-\ell^+\ell^-$ decays comprising $\Lambda$ resonances with spin up to $\leq5/2$

This paper describes the angular distribution of $\Lambda_b^0\to \Lambda(\to pK^-)\ell^+\ell^-$ decays. A full expression is given for the case of multiple interfering spin-states with spin $\leq \tfrac{5}{2}$. This distribution is relevant for future measurements of $\Lambda_b^0\to pK^-\ell^+\ell^-$ decays, where different states cannot easily be separated based on their mass alone. New observables arise when considering spin-$\tfrac{5}{2}$ states as well as interference between states. An exploration of their behaviour for a variety of beyond the Standard Model scenarios shows that some of these observables exhibit interesting sensitivity to the Wilson coefficients involved in $b\to s\ell^+\ell^-$ transitions. Others are insensitive to the Wilson coefficients and can be used to verify the description of $\Lambda_b^0\to \Lambda$ form-factors. A basis of weighting functions that can be used to determine all of the angular observables described in this paper in a moment analysis of the experimental data is also provided.

==> moments/K10.tex <==
K_{10} = \frac{1}{15\sqrt{21}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+6\sqrt{3} \left(
  \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{-}
+ \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-} \right. \\
&\left.- \sqrt{3} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
 \right) + \left(\frac{5}{2}\longleftrightarrow \frac{3}{2}\right) \\
&+ 15\sqrt{3}\lambda \left(
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{-}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-}
 \right) + \left(\frac{5}{2}\longleftrightarrow \frac{1}{2}\right) \\
&+2\lambda  \left(
+ 4 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{-}
+ 4 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ 7 \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\right) \\
&+9\lambda \left(
+3 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{-}
+3 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
-  \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right)\Big] \\
&+\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K11.tex <==
K_{11} = \frac{1}{15\sqrt{7}}\sum_{\lambda=\pm1}\text{Re}\Big[
%
&6\sqrt{3}\lambda\left(- \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ \sqrt{3} \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) + \left(\frac{3}{2}\longleftrightarrow \frac{5}{2}\right) \\
%
&- 15 \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-}
+ \left(\frac{1}{2}\longleftrightarrow \frac{5}{2}\right) \\
%
&- 27 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+  9 \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-} \\
%
&-  8 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 14 \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}\Big] \\
&+ \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K12.tex <==
K_{12} = \frac{1}{30\sqrt{105}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+6 \sqrt{3} \left(
- 2 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{-}
-   \sqrt{3} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}\right. \\
&\left.+   \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-} \right)
+ \left(\frac{5}{2}\longleftrightarrow \frac{3}{2}\right) \\
&+15 \sqrt{3}\lambda \left(
+  \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-}
-2 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{-} \right)
+ \left(\frac{5}{2}\longleftrightarrow \frac{1}{2}\right) \\
&+9\lambda \left(
-  \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+3 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
-6 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{-}
\right) \\
&+ 2\lambda \left(
-8 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{-}
+4 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+7 \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\right)\Big] \\
&+\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K13.tex <==
K_{13} = \frac{1}{7 \sqrt{3}}
\sum_{\lambda=\pm1}
4\lambda
\text{Re}\Big[
&+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+}
+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
-         \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\Big] \\
&- 3 \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
+ 2 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+}\Big|^2
+ 2 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2 \\
&+\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K14.tex <==
K_{14} = \frac{1}{7}\sum_{\lambda=\pm}
\text{Re}\Big[
&- 2 \sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ 2 \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+\left(\frac{3}{2}\longleftrightarrow \frac{5}{2}\right) \\
&-2\lambda \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
+3\lambda \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \Big] \\
&+ \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K15.tex <==
K_{15} = \frac{1}{7\sqrt{15}}\sum_{\lambda=\pm1}&\Big(2\lambda\text{Re}\Big[
- 2 \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+}
+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
- \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\Big]\Big) \\
&- \frac{3}{2} \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
- 2 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+}\Big|^2
+ \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2 \\
&+\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K16.tex <==
K_{16} = 
\frac{25}{21\sqrt{33}}&\sum_{\lambda=\pm1} \lambda\text{Re}\Big[
+ 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-}
+ 2 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-} \Big] \\
+&\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K17.tex <==
K_{17} = \frac{25}{21 \sqrt{11}}&\sum_{\lambda=\pm1}\text{Re}\left[
\AmpJP{V*}{\frac{3\lV}{2}}{\lV}{\frac{5}{2}}{{{-P}}} \AmpJP{A}{\frac{3\lV}{2}}{\lV}{\frac{5}{2}}{P} - 2 \AmpJP{V*}{\frac{\lV}{2}}{\lV}{\frac{5}{2}}{{{-P}}} \AmpJP{A}{\frac{\lV}{2}}{\lV}{\frac{5}{2}}{P}
\right]+ \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K18.tex <==
K_{18} = \sqrt{\frac{5}{33}}\frac{5}{42}&\sum_{\lambda=\pm1}\lambda
\text{Re}\Big[
- 4 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-}
+ 2 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-} \Big] \\
+&\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K19.tex <==
K_{19} =
\frac{1}{35\sqrt{30}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+21\left(
- \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+          \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) \\
&+ 21 \sqrt{3} \left(\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
\right)
-\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
&- 35 \left(
\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+ \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right)
-\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right) \\
&+ 7 \sqrt{2}\lambda \left(
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+ \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) \\
&+ 3\lambda \left(
4 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3\lambda}{2}}{\lambda}{\frac{5}{2}}{-}
- 3 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right) \\
&- 35 \sqrt{2}\lambda  \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{1}{2}}{-}
\Big] \\
&+ \left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K20.tex <==
K_{20} =
\frac{1}{35\sqrt{6}}
\sum_{\lV=\pm1}
\text{Re}\Big[
&- 35\sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{1}{2}}{-} \\
%
&- 7 \sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
- 14\sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-} \\
%
&- 12        \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 9\sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-} \\
%
&+21\lambda\left(
+ \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
- \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-} \right. \\
&\left.-          \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ \sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\right) \\
%
&+35\lambda\left(
- \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+ \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right)
-\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)
\Big] \\
%
+&\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K21.tex <==
K_{21} =
\frac{1}{35\sqrt{2}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+ \sqrt{2}  \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
- 5         \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+} \\
&- 5         \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+ 3 \sqrt{3}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \\
&- 7\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
- 4\sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
&- 7\sqrt{2} \left(
\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}\right)
-\left(\frac{5}{2}\longleftrightarrow\frac{1}{2}\right) \\
%
&-7\lambda\left(
\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)
\Big] \\
&+ \left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K22.tex <==
K_{22} =
-\frac{1}{7\sqrt{10}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&- 4 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
- 7 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \\
%
&+ 3\lambda \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{2}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&+ 5\lambda \left(\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{A}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+ 7 \sqrt{2}\left( \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{A}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
-\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\right)
- \left(\frac{5}{2}\longleftrightarrow\frac{1}{2}\right) \\
%
&+ 7\lambda \left(\sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{A}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
- \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{A}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)
\Big] \\
%
+&\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda) \,,

==> moments/K23.tex <==
K_{23} =
\frac{1}{5\sqrt{210}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&- 5\sqrt{6}\lambda\left(
\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right)
+\left(\frac{1}{2}\longleftrightarrow\frac{5}{2}\right) \\
&+\lambda\left(
- 8 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
- 18 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}\right. \\
%
&+ \left.2\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 6\sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) \\
&+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
-\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&- 7 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 9 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\Big] \\
&+ \left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K24.tex <==
K_{24} =
\frac{1}{5\sqrt{42}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+\sqrt{6} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
-\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+ 7\sqrt{3} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ 9\sqrt{2} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-} \\
%
&+\left(
- 10 \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
+ 5\sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\right)
+\left(\frac{5}{2}\longleftrightarrow\frac{1}{2}\right) \\
%
&- 18 \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+ 6 \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-} \\
%
&+\left(
- 2\sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 8 \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)
\Big] \\
%
+&\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda) \,,

==> moments/K25.tex <==
K_{25} =
-\frac{1}{7}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+\lambda \left( \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{\frac{3}{2}} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right) \\
%
&+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&+\sqrt{3}\lambda  \left(
\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda,}{\lambda}{\frac{5}{2}}{+}
\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right)\Big] \\
&+ \left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K26.tex <==
K_{26} =
\frac{1}{7}\sqrt{\frac{5}{2}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+ \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
&+\sqrt{2}\lambda  \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&-\sqrt{6}\left(
\AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)
\Big] \\
%
&+\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda) \,,

==> moments/K27.tex <==
K_{27} =
-\frac{10}{7\sqrt{66}}
\sum_{\lambda=\pm1}
\lambda\text{Re}\Big[
&\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}\Big] \\
&+ \left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K28.tex <==
K_{28} =
\frac{5}{7}\sqrt{\frac{10}{33}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&- \sqrt{2}\AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
+ \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\Big] \\
%
+&\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K29.tex <==
K_{29} =
-\frac{1}{35\sqrt{30}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&+35\lambda\left(
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
- \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right)
-\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right) \\
%
&+21\lambda\left(
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
-\sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}\right. \\
%
&+\left.
+\sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right) \\
%
&+ 12        \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ 9\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-} \\
%
&+ 35\sqrt{2}\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{1}{2}}{-} \\
%
&+ 7\sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ 14\sqrt{2}\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
\Big] \\
%
&+\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K30.tex <==
K_{30} =
-\frac{2}{70\sqrt{6}}
\sum_{\lambda=\pm1}
\text{Im}
\Big[
&+7\sqrt{2} \lambda\left(
2 \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
- \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) \\
%
&+\lambda\left(
9 \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
-2 \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
\right) \\
%
&+ 35 \sqrt{2} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{1}{2}}{-} \\
%
&+ 35\left(
\sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
\right)
-\left(\frac{1}{2}\longleftrightarrow\frac{3}{2}\right) \\
%
&+ 21 \sqrt{3} \left(
\AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right)
-\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+ 21 \left(
\sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right)
\Big] \\
%
&+\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right)\,,

==> moments/K31.tex <==
K_{31} = -\frac{1}{70}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&-\lambda\left( 7 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ 4 \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\right) \\
%
&+ 3 \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&+ 5\sqrt{2} \left(\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&- 14\lambda \left(
    \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
 + \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{1}{2}}{+}
\right)
-\left(\frac{1}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+7 \sqrt{2}\left(
- \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
\right)
+\left(\frac{3}{2}\longleftrightarrow\frac{1}{2}\right)\Big] \\
%
&+\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right)\,,

==> moments/K33.tex <==
K_{33} = -\frac{1}{5\sqrt{210}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&+ \lambda \sqrt{6} \left(-\AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{-} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}\right) \\
&- 9 \sqrt{2} \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
- 7 \sqrt{3} \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{-} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&- 6 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{-} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ 18 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{-} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+} \\
%
&+ 5\sqrt{6} \left(
\sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{-} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
- \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{-} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right)
+\left(\frac{1}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+ 2 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
+ 8 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{-} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+} \Big] \\
%
+&\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K34.tex <==
K_{34} = -\frac{1}{5\sqrt{42}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&5 \sqrt{6} \lambda \left(
\AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right)
+\left(\frac{1}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
+ &\sqrt{6} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
-\left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
+ &9 \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ 7 \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-} \\
%
+ &2 \sqrt{2} \lambda \left(
- \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ 2 \sqrt{2} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
\right) \\
%
+ &6 \sqrt{3} \lambda \left(
+ \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+ \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
\right) \Big] \\
%
+&\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K35.tex <==
K_{35} = -\frac{\sqrt{2}}{14}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&- \sqrt{2} \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&- \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
- \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \\
%
&+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
+ \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
 \Big] \\
%
+&\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K36.tex <==
K_{36} = -\frac{\sqrt{5}}{7\sqrt{2}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&+\lambda\left(
  \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right) \\
%
&+\sqrt{6}\lambda\left(
 \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V*}{-\frac{1}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
\right)
+ \left(\frac{3}{2}\longleftrightarrow\frac{5}{2}\right) \\
%
&+ \sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
 \Big] \\
%
+&\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K37.tex <==
K_{37} = -\frac{10}{7\sqrt{66}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&+ \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
- \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
 \Big] \\
%
+&\left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K38.tex <==
K_{38} = -\frac{10}{7}\sqrt{\frac{10}{33}}
\sum_{\lambda=\pm1}
&\text{Im}\Big[
+\sqrt{2} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{1}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
+\lambda \AmpJP{A*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K39.tex <==
K_{39} = \frac{1}{35}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&-6 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
-7 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+} \\
&+4 \sqrt{2}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
-2 \sqrt{3}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+} \\
&+7 \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+14\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K40.tex <==
K_{40} = \frac{1}{15 \sqrt{7}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+2 \sqrt{3}\lambda  \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
+9 \sqrt{2}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{-} \\
%
&
+15 \lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-} \\
&-6 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
-3 \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K41.tex <==
K_{41} = \frac{1}{7}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&-                \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+ \sqrt{6}\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+2 \lambda       \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K42.tex <==
K_{42} = \frac{5}{\sqrt{231}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
 \Big] + \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K43.tex <==
K_{43} = \frac{1}{35}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&-6 \lambda \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
-7\lambda \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+} \\
&+14                \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
+7 \lambda         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+} \\
&-2 \sqrt{3}         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
+4 \sqrt{2}         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K44.tex <==
K_{44} = \frac{1}{15 \sqrt{7}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&-3 \lambda \sqrt{2} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
-6 \lambda \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{-} \\
%
&+15                \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-} \\
%
&+9 \sqrt{2}         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{-}
+2 \sqrt{3}         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K45.tex <==
K_{45} = \frac{1}{7}
\sum_{\lambda=\pm1}
\text{Im}\Big[
&-\lambda         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+        \sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{+}
+        2       \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{3}{2}}{+}
 \Big] \\
&+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,,

==> moments/K46.tex <==
K_{46} = \frac{5}{\sqrt{231}}
\sum_{\lambda=\pm1}
\text{Im}\Big[
\AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{-\frac{3}{2}\lambda}{-\lambda}{\frac{5}{2}}{-}
 \Big]
+ \left(V\longleftrightarrow A\right)
+\left(\pLambda\longrightarrow-\pLambda\right) \,.

==> moments/K5.tex <==
K_5 = -\frac{2}{5\sqrt{3}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
+ \frac{1}{14} &\left(
   9 \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+  3 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}\right. \\
&\left.+ 21 \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+  7 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}\right. \\
&\left.+ 35 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-} \right)\\
%
+\frac{1}{\sqrt{2}}\lambda  &\left(
 3 \sqrt{2} \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ 3 \sqrt{3} \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+ \left(\frac{5}{2}\longleftrightarrow \frac{3}{2}\right)\right. \\
%
&\left.+ 5 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+ \left(\frac{1}{2}\longleftrightarrow \frac{3}{2}\right)
\right) \Big] \\
&+ \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K6.tex <==
K_6 = \frac{1}{30\sqrt{5}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+ 3 \sqrt{2} \left(
    \sqrt{2} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+   \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}\right. \\
&\left.- 2 \sqrt{3} \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{-}
\right)
+ \left(\frac{3}{2} \longleftrightarrow \frac{5}{2}\right) \\
&+ 5 \sqrt{2} \left(
+   \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-}
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{-}
\right) + \left(\frac{1}{2}\longleftrightarrow \frac{3}{2}\right) \\
&+ 5 \lambda \left(
+   \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{-}
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{-}
\right) \\
&+\lambda \left(
+ 3 \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
+   \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{-}
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{-}
\right) \\
&+ \frac{3}{7} \lambda \left(
+ 3 \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
+   \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{-}
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{-}
\right)\Big] \\
&+\left(V\longleftrightarrow A\right) + (\pLambda\longrightarrow -\pLambda)\,,

==> moments/K7.tex <==
K_7 = \frac{2}{7\sqrt{15}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+ \lambda \sqrt{6} \left(
+         \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+}
+         \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
+ \sqrt{6} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right) \\
&+7 \sqrt{3} \left(
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right) \\
&+ 7 \lambda \sqrt{2} \left(
+ \AmpJP{V*}{\frac{1}{2}\lambda}{0      }{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+}
+ \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
\right)\Big] \\
&+\frac{7}{2}\left(
+ \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{3}{2}}{+}\Big|^2
+ \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\Big|^2
- \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\Big|^2
\right) \\
&+\left(
+ 4 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0      }{\frac{5}{2}}{+}\Big|^2
+ 4 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
+   \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
\right) \\
&+\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K8.tex <==
K_8 = \frac{1}{7\sqrt{5}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&- 7\sqrt{2} \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+}
+ \left(\frac{3}{2}\longleftrightarrow \frac{1}{2}\right) \\
&- 7 \sqrt{3} \lambda \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+}
+ \left(\frac{5}{2}\longleftrightarrow \frac{1}{2}\right) \\
&- \sqrt{6} \left(
+         \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{6} \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
\right) + \left(\frac{3}{2}\longleftrightarrow \frac{5}{2}\right)\\
&+7\lambda \left(
- \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \right) \\
&+2\lambda \left(
- 4 \AmpJP{A*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
-   \AmpJP{A*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}
\right)\Big] \\
&+ \left(\pLambda\longrightarrow -\pLambda\right)\,,

==> moments/K9.tex <==
K_9 = \frac{1}{35\sqrt{6}}
\sum_{\lambda=\pm1}
\text{Re}\Big[
&+ 7\sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+}
- 14\sqrt{6} \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \\
&+ 14\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{1}{2}}{+}
- 28\lambda \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{1}{2}}{+} \\
%
&+ 2\sqrt{3}\lambda \left(
\AmpJP{V*}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
+ \sqrt{6} \AmpJP{V*}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+} \AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}
- 2 \AmpJP{V*}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+} \AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+}\right)
\Big] \\
%
&+ \frac{7}{\sqrt{2}}\left(
+ \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\Big|^2
- \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{3}{2}}{+}\Big|^2
- 2 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{3}{2}}{+}\Big|^2
\right) \\
&+ \sqrt{2}\left(
- 8 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{0}{\frac{5}{2}}{+}\Big|^2
+ 4 \Big|\AmpJP{V}{\frac{1}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
+ \Big|\AmpJP{V}{\frac{3}{2}\lambda}{\lambda}{\frac{5}{2}}{+}\Big|^2
\right) \\
&+\left(V\longleftrightarrow A\right) + \left(\pLambda\longrightarrow -\pLambda\right)\,,
